Investigating Exploratory Search Activities based on the Stratagem Level in Digital Libraries

In this paper we present the results of a user study on exploratory search activities in a social science digital library. We conducted a user study with 32 participants with a social sciences background -- 16 postdoctoral researchers and 16 students -- who were asked to solve a task on searching related work to a given topic. The exploratory search task was performed in a 10-minutes time slot. The use of certain search activities is measured and compared to gaze data recorded with an eye tracking device. We use a novel tree graph representation to visualise the users' search patterns and introduce a way to combine multiple search session trees. The tree graph representation is capable to create one single tree for multiple users and to identify common search patterns. In addition, the information behaviour of students and postdoctoral researchers is being compared. The results show that search activities on the stratagem level are frequently utilised by both user groups. The most heavily used search activities were keyword search, followed by browsing through references and citations, and author searching. The eye tracking results showed an intense examination of documents metadata, especially on the level of citations and references. When comparing the group of students and postdoctoral researchers we found significant differences regarding gaze data on the area of the journal name of the seed document. In general, we found a tendency of the postdoctoral researchers to examine the metadata records more intensively with regards to dwell time and the number of fixations.

==> methodandDemographics.tex <==
\section{User Study}\label{methodandsetup}
\subsection{Setup}
The user study took place in single sessions in obne of our labs with a duration of about 30 minutes each. We made sure that the conditions were the same in each session: The experiment was run on a laptop connected to an external 22''-monitor as the stimlulus monitor for the participants. An additional keyboard and a mouse were attached to the laptop as controlling devices. The display of the laptop was used for observation. We used an SMI iView Remote Eye tracking Device 250 that was installed at the bottom of the stimulus monitor. The screen activities as well as the eye movements were recorded by the corresponding software SMI Experiment Suite 360°. We used a nine point calibration with a both visual and quantitative validation to make ensure the quality of the gaze data and defined a sampling frequency of 250Hz for recording the eye movements. All participants used Mozilla Firefox for solving the task.


\subsection{Scenario}
All participants had to accomplish the same task shown in \ref{fig:scenario}.
\begin{figure}
	\begin{center}
		\begin{center}
			\includegraphics[trim=60 510 285 70,clip, width=1.0\linewidth]{figures/Task.pdf}
		\end{center}
		\caption{The scenario for the user study.}
		\label{fig:scenario}
	\end{center}
	\vspace{0.0em}
\end{figure}
They started with the same document titled \em ethnical education inequality at start of school \em and had a limit of ten minutes to solve the task. Having to use Sowiport \cite{Hienert2015} for their literature search, the participants had access to about 9 million documents of the social sciences from 18 different databases of which six are English-language ones. 
The seed document (see Figure \ref{seeddocdesc}) was published by two authors, consisted of five keywords and one classification and was published in a german journal for sociology and social psychology. Each of these informations were implemented as hyperlinks and could be utilized for further exploration.  In separat tab views the participants could browse through citations (four citations all accessible in Sowiport via hyperlinks), reference information (70 citations of which 33 are accessible in Sowiport via hyperlinks) and read the abstract of the given seed document. Additionaly the participants had access to the full text of the seed document. Besides these informations the authors were provided with ten recommendations. Five provided by the SOLR \em more like this function \em and the remaining five were associated documents that were published in the same journal. As Sowiport comprises 18 different databases it is possible that duplicate documents are recommended.

\begin{figure*}[htbp]
	\subfloat[Seed document] {\includegraphics[width=1\linewidth]{figures/seed.png}}
	\vspace{\fill}
	\subfloat[Citation tab] {\includegraphics[width=0.45\linewidth]{figures/seed_cite.png}}
	\hspace{\fill}
	\subfloat[Reference tab]{\includegraphics[width=0.45\linewidth]{figures/seed_ref.png}}
	\hspace{\fill}
	\caption{Seed document for the user study.}
	\label{fig:seeddocdesc}
\end{figure*}



\subsection{Procedure}
The user study was divided into three parts. Each session followed a detailed protocol to make sure that the conditions were the same for each participant. After a short introduction to the background of the study and the procedure, each participant signed a consent form about the recording of the gaze data as well as the screen activities. 

In the first part of the study, the participants were handed out a pre-questionnaire consisting of seven questions that covered demograhic information as well as their search experience in DLs. Regarding their search experience on five point scales we asked for the participant's overall use of digital libraries (1=very rarely; 5=very often) and the use of the three digital libraries ACM DL, Web of Science and Sowiport in particular as well as Google Scholar (1=very rarely; 5=very often). 

In the second and main part of the user study the participants were provided with the scenario and the task they had to solve. For this, the eye tracking technology as well as the task were shortly explained. The participants were asked to take an upright and comfortable sitting position in order to move as little as possible during the search task. Then the monitor with the eye tracker was aligned to their height and eye level so that their eyes were positioned in the center of the area the eye tracker captures. The eye tracker was calibrated and only if the result was good or very good the experiment was started. The participants were first displayed te scenario. After reading, they proceeded to the start document for the search task in Sowiport by pressing the space bar. While the participants were solving the task, we observed their activities and eye movements on the observation screen and noted down which stratagems they used and which information they looked at. We focused on the six stratagems that were derived from \cite{Bates:79} and that we had already used in the survey. After ten minutes, the participants were told to end their search and review the documents they had collected in browser tabs. They were allowed to close the documents they do not consider relevant any more.

In the third and last part of the session the subjects had to fill out a questionnaire covering five questions about the task in general that mostly had to be answered on five point scales: How would you consider the difficulty of the given task overall (1=very easy; 5=very difficult)? How difficult was it to find relevant documents (1=very easy; 5=very difficult)? How would you rate the system's ability at providing you with relevant documents (1=not good; 5=very good)? How successful was your search (1=unsuccessful; 5=successful)? Which part of solving the task would you consider particularly difficult and why? Furthermore they had to answer questions about their use of stratagems that were based on the observations we made during the search task. One the one hand we asked the participants to state the reasons for their use of a stratagem, rate their usefulness on a five point scale and justify their usefulness rating:
\begin{itemize}
\item You solved the task by following the references of the document.
\begin{itemize}
\item Why did you choose this method?
\item How useful was this method? (1=not at all useful, 5=very useful)
\item Please give reasons for your choice of usefulness.
\end{itemize}
\end{itemize}
On the other hand we asked why they had looked at a particular information but decided not to use it as a search method:
\begin{itemize}
\item You looked at the classification terms of a document but did not follow them.
\begin{itemize}
\item Why didn’t you use this method?
\end{itemize}
\end{itemize}
After filling out the questionnaire the session was ended and the participants were thanked.

\section{Methodology}

We examined the results of our user study using screen casts, eye tracking data and network analysis each \\method addressing one of the research questions described in Section \ref{RQINTRO}. To quantify the usage frequency of search activities we examined the screen casts of the participants. Besides the general usage of search activities we utilized eye tracking data to gain information on the implicit usefulness of search activities. To analyze the eye tracking data we exploit heath maps to get a visual representation of the participants gaze data and areas of interest (aoi) to quantify and compare potential search activities. The results of the usage frequencies and the eye tracking experiment are presented in Section \ref{descriptive} and address the first research question.

In Section \ref{graphs} we present the results of our network analysis in which the search activities of each participant are transformed into a tree graph representation. Given the tree graph we address the second research question: We build a tree graph representation that is shared by most participants to get a visual representation of the most common. Out of the tree graph we derive different features (e.g. diameter..) and use machine learning? 

In Section \ref{eyetracker} we compare the results of the usage frequency and the network analysis between the two groups of participants. To seek for significant difference in the search behaviour we utlize a non-parametric Mann-Whitney test ($\alpha$ $\le$ 0.05).
  
For each participant, full screen records were taken during the search task that showed their gaze data and also captured the navigation bar of the web browser as well as overlaying dynamic elements. We used these records to reproduce the user journey of each participant. The used stratagems, the collected relevant documents and the deleted documents per stratagem were counted. 

For analysing the participants' gaze data we prepared the data in three steps: First, we defined a fixation time threshold of 104ms, since this time marks the start of lexical processing \cite{reichle2012using}. Second, for each participant we determined the stable eye by comparing the scanpaths of the left and the right eye of a participant in order to minimize divergences. Third, we reduced the data to three stimuli -- the start document, the reference list of the start document and the citation list of the start document -- and the first visit on each of these stimuli. We focused on the timespan between entering the document and the first interaction with a clickable object. Thus, overlaying elements such as the search term recommender that would have distorted the gaze data were eliminated.

We created heat maps and defined areas of interest (AOIs) for each of the stimuli. For determining statistical significance, we used XYZ with

\subsection{Pattern analysis}\label{graphs}

In order to address our second research Question, we need a way to analyse our participants' session on a structural bases. Therefore, we create trees as a structural representation of our participants' search sessions. To illustrate how we create such session trees, Figure \ref{fig:tree_examples} shows three fictitious examples of session trees and the corresponding search patterns. In the first session, starting from the root document, the document's citations were clicked and one of the cited documents visited. This is represented by the left two nodes in session tree \ref{fig:tree_examples}a. After that, the user returns to the citations list and then to the root document. As this only involves already visited pages, it does not result in additional nodes. At the end of the session, the user conducts a search, which accounts for the right node in session tree a.

\begin{figure}[htbp]
	\subfloat[session 1]{\includegraphics[width=0.31\linewidth]{figures/graph/example_1.png}}
	\subfloat[session 2]{\includegraphics[width=0.31\linewidth]{figures/graph/example_2.png}}
	\subfloat[session 3]{\includegraphics[width=0.31\linewidth]{figures/graph/example_3.png}} \\
	\begin{itemize}[align=left,
		leftmargin=2em,
		itemindent=0pt,
		labelsep=0pt,
		labelwidth=2em]
		\item[\textbf{Session 1: }]  $doc_{root} \rightarrow citation \rightarrow doc_1 \rightarrow citation  \rightarrow doc_{root} \rightarrow search$	\\	
		\item[\textbf{Session 2: }] $doc_{root} \rightarrow journal \rightarrow doc_{root} \rightarrow author \rightarrow doc_1 \rightarrow author \rightarrow doc_2$	\\
		\item[\textbf{Session 3: }]  $doc_{root} \rightarrow search \rightarrow doc_1 \rightarrow search \rightarrow doc_2 \rightarrow search \rightarrow doc_{root} \rightarrow journal \rightarrow doc_{root} \rightarrow citation \rightarrow doc_3$	
	\end{itemize}
	\caption{Session tress (a-b) for three example search session (1-3)}
	\label{fig:tree_examples}
\end{figure}

For this representation, ignore the type of the nodes. The information whether a node represents a document, a search, or a citation list is discarded. Also, we treat the usage of recommendations equal to other stratagems. Meaning, that if at least one recommendation is clicked, we insert a node representing the list of recommendations and a child node for each clicked recommendation, although no extra click is needed to display the list of recommendations. Furthermore, we discard the order of the search session. Instead, we sort the tree by subtree size from left to right. Therefore, on one level, nodes with more subnodes are sorted further to the left than those with less subnodes. This can be observed in session 2 of figure \ref{fig:tree_examples}. The usage of the author stratagem appears after the journal usage, but the corresponding nodes are on the left side, because there are more sub sequential actions involved.

\begin{comment}
Session trees allow a structural overview over the way in which a participant searched. One can see whether the participant inspects a few lists of documents intensely (e.g. a search result list or the citations list), by clicking on many documents or prefers to browse less through a higher amount of different lists, while only investigating a smaller share of documents. \todo{reference to exhaustive and explorative users}. 
\end{comment}

To extend the analysis from individuals to groups of participants and thus, to understand and find common patterns, we need a way to combine multiple session trees into one conjoint tree. To do this, we have implemented a tool, with which we combine the session trees.\footnote{Upon acceptance, we will publish the tool and the participants' trees as open source on github.} Instead of combining all trees at once, we merge pairs of trees iteratively. We start with an empty tree and merge it with the first session tree. The resulting tree is then merge with the next tree and so forth. Figure \ref{fig:tree_examples_merged}a shows the merged tree of the examples session tree 1 (cf. Figure \ref{fig:tree_examples}a) and session tree 2 (cf. Figure \ref{fig:tree_examples}b). When two nodes are merged, the weights of their edges are summed up. After merging session tree 1 and 2, we merge the resulting tree with the tree of session 3 (cf. Figure \ref{fig:tree_examples}c), shown in Figure \ref{fig:tree_examples_merged}b.

\begin{figure}[htbp]
	\hspace{\fill}
	\subfloat[session 1 and 2 merged] {\includegraphics[width=0.31\linewidth]{figures/graph/example_merged_1-2.png}}
	\hspace{\fill}
	\subfloat[session 1, 2, and 3 merged]{\includegraphics[width=0.31\linewidth]{figures/graph/example_merged_1-2-3.png}}
	\hspace{\fill}
	\caption{Merging of session trees}
	\label{fig:tree_examples_merged}
\end{figure}

When merging two trees, one has to decide which nodes have to be merged. As each node and its child nodes are an individual tree, this decision has to be made recursively on each level of the trees. For each pair of nodes on one level, we create all possible combinations of subtrees and select the best combination along two conditions. First, the number of nodes in the resulting subtree has to be minimal. Second, the weight of the subtree has to be optimized. For the second condition we needed to define what is a weight of a subtree and what is an optimum for the subtree weight.

\todo{formel subtree weight}

\todo{optimum of subtree weight}

Following the described procedure, we receive exactly one resulting tree, when combining two session trees. However, when merging multiple trees iteratively, the resulting tree depends on the order in which the trees are merged. If merging two specific nodes result in an maximal subtree weight, is depended on in how far the resulting node can be merged efficiently with node of the following trees. To find the optimal merging order, we would need to calculate all possible permutations, in which the session trees could be merged. This would result in $32! \approx 2,63 \mathbin{\times} 10^{35}$ merging orders for the complete set of trees in our study. As this exceeded our computational capacities for this paper, we decided to use another approach. When sorting the session trees in ascending order of their root nodes subtree weight, the resulting trees slowly increase in weight (in general trees with a small subtree weight tend to be more compact trees). In this way, common structures, that exist in many trees are merged very early, whereas outliers are merged later. The sorting does not guarantee an optimal merging order! However, it ensures, that there is only one resulting tree for a set of trees and that all combined trees are created with the same procedure. We believe, that sorting the trees results in a sub optimal tree, that is close enough to the optimal tree, to allow to draw meaningful conclusions for our analysis.



\section{Demographics}\label{demographics}%müsste eig unterpunkt des kapitels sein
The user study involved 32 participants that were divided into two groups A and B. While group A included 16 students, group B consisted of 16 postdoctoral researchers. All participants were social scientists from different fields of study that had been recruited via e-mail and personal recommendation.

The students were aged 22 to 35 years (avg=26.38, sd=3.76). 75\% were female and 25\% male. About 19\% of the students had no academic degree yet, 69\% held a bachelor's degree, 15\% held a master's degree and 6\% had a diploma.
The postdoctoral researchers' age was slightly higher and ranged from 30 to 62 (avg=40.19, sd=9.23). In this group, 50\% were female and 50\% male.

The participants were asked about their search expertise, in particluar their experience in searching digital libraries and rated it on five point  scales (1=none at all, 5=expert).
Regarding their overall search experience in digital libraries, 25\% of the students stated to have little experience, 56\% rated their experience as moderate and 19\% considered their experience high, resulting in an average search experience of 2.94 (sd=0.66). In contrast, 38\% of the postdocs considered their experience little and 31\% moderate, while 25\% stated to have a high or expert experience, with an average search experience of 2.88 (sd=1.11).

In accordance with the online survey, on a five point scale (0=very rarely, 5=very often) we asked the participants about their use of digital libraries and Google Scholar. In the students' group, 5\% stated that they used DLs in general often or very often (avg=2.88, sd=0.99). 25\% indicated to use Sowiport often or very often (avg=2.81, sd=1.07) and 62.5\% used Google Scholar often or very often (avg=3.69, sd=0.92). Out of the postdocs, %sacht mer das so?
19\% used DLs in general often or very often and 6\% stated to use Sowiport often or very often, while 63\% claimed to use Google Scholar often or very often. 
[sind hier web of science und andere DLs auch noch interessant? kann die mit angeben wenn ich soll. dachte nur, ich halte es fokussiert.]

